Pronunciation Deviation Analysis Through Voice Cloning and Acoustic Comparison

This paper presents a novel approach for detecting mispronunciations by analyzing deviations between a user's original speech and their voice-cloned counterpart with corrected pronunciation. We hypothesize that regions with maximal acoustic deviation between the original and cloned utterances indicate potential mispronunciations. Our method leverages recent advances in voice cloning to generate a synthetic version of the user's voice with proper pronunciation, then performs frame-by-frame comparisons to identify problematic segments. Experimental results demonstrate the effectiveness of this approach in pinpointing specific pronunciation errors without requiring predefined phonetic rules or extensive training data for each target language.

==> algo.tex <==
\subsection{Algorithm}

\begin{breakablealgorithm}
\caption{Mispronunciation Detection via TTS‐Clone Comparison}
\begin{algorithmic}[1]
\Require Real utterances $U=\{u_i\}_{i=1}^M$, base TTS model $V$, significance levels $\alpha_C,\alpha_I$, Class‐specific thresholds $\tau_C,\tau_I$ and mispronunciation labels for new utterances 
\State \textbf{Calibration phase:}
\For{$i \leftarrow 1$ \textbf{to} $M$}
  \State $\hat u_i \leftarrow V(u_i)$  \Comment{Speaker‐adapted TTS clone}
  \State Extract word alignments 
    $\{(w_j,[s_j^{\mathrm{real}},e_j^{\mathrm{real}}],[s_j^{\mathrm{clone}},e_j^{\mathrm{clone}}])\}_j$
  \For{each aligned token $w_j$}
    \State Extract MFCC envelopes $E_j^{\mathrm{real}},E_j^{\mathrm{clone}}$
    \State Compute DTW distance 
      $d_j^{\mathrm{DTW}} = \min_{\pi}\sum_t\|e_{j,t}^{\mathrm{real}}-e_{j,\pi(t)}^{\mathrm{clone}}\|$
    \State Normalize: $\bar d_j \leftarrow d_j^{\mathrm{DTW}} \;/\; \max_t|u_i(t)|$
    \State Append $\bar d_j$ to $\mathcal{D}_{\text{correct}}$ or $\mathcal{D}_{\text{incorrect}}$ by true label
  \EndFor
\EndFor
\State Compute thresholds:
  \[
    \tau_C \leftarrow \text{Percentile}(\mathcal{D}_{\text{correct}},\,1-\alpha_C),\quad
    \tau_I \leftarrow \text{Percentile}(\mathcal{D}_{\text{incorrect}},\,1-\alpha_I)
  \]
\hrulefill
\State \textbf{Detection phase (new utterance $u$):}
\State $\hat u \leftarrow V(u)$
\State Repeat alignment, feature extraction, distance computation to obtain $\{\bar d_j\}$
\For{each word $w_j$ with distance $\bar d_j$}
  \State Compute empirical CDFs:
    $p_C \leftarrow F_{\text{correct}}(\bar d_j)$,
    $p_I \leftarrow F_{\text{incorrect}}(\bar d_j)$
  \State Compute median‐distances:
    $\delta_C \leftarrow |p_C-0.5|$,\;
    $\delta_I \leftarrow |p_I-0.5|$
  \State Select distribution:
    \[
      D^* \leftarrow
      \begin{cases}
        \text{correct}, & \delta_C < \delta_I,\\
        \text{incorrect}, & \text{otherwise.}
      \end{cases}
    \]
  \State Set threshold $\tau^* \leftarrow
    \begin{cases}
      \tau_C, & D^*=\text{correct},\\
      \tau_I, & D^*=\text{incorrect}
    \end{cases}$
  \State Assign label:
    \[
      \hat y_j \leftarrow
      \begin{cases}
        \text{CORRECT},   & D^*=\text{correct}\ \land\ \bar d_j \le \tau_C,\\
        \text{INCORRECT}, & D^*=\text{incorrect}\ \land\ \bar d_j \ge \tau_I,\\
        \text{AMBIGUOUS}, & \text{otherwise}.
      \end{cases}
    \]
\EndFor
\end{algorithmic}
\end{breakablealgorithm}


==> methods.tex <==

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\real}{\mathrm{real}}
\newcommand{\clone}{\mathrm{clone}}
\newcommand{\correct}{\mathrm{correct}}
\newcommand{\incorrect}{\mathrm{incorrect}}
\section{Methodology}
The mispronunciation detection system operates through two phases: \textit{calibration} (model training) and \textit{runtime} (deployment). We define the core mathematical framework as follows.

\subsection{Problem Formulation}
Let $\mathcal{U} = \{u_i\}_{i=1}^N$ be a corpus of real speech utterances with TextGrid annotations. Each utterance $u_i$ generates a synthesized clone $\hat{u}_i = V(u_i)$ via TTS system $V$. For each word $w_j$ in utterance $u_i$, we have ground truth label $y_j \in \{\correct, \incorrect\}$.

\subsection{Calibration Phase}
\vspace{-0.5em}
\begin{align}
&\mathbf{\Phi} = \{(u_i, \hat{u}_i, \mathcal{W}_i, Y}_{i=1}^N \quad \text{(Training corpus)} \\
&\mathcal{W}_i = \bigl\{\bigl( w_j,\, [s_j^{\real}, e_j^{\real}],\, [s_j^{\clone}, e_j^{\clone}] \bigr) \bigr\}_{j=1}^{M_i} \quad \text{(Word alignment)} \\
&\mathbf{E}_j^{\real} = \Psi\bigl(u_i(s_j^{\real}:e_j^{\real})\bigr) \in \mathbb{R}^{13 \times T_j^{\real}} \quad \text{(MFCC features)} \\
&\mathbf{E}_j^{\clone} = \Psi\bigl(\hat{u}_i(s_j^{\clone}:e_j^{\clone})\bigr) \in \mathbb{R}^{13 \times T_j^{\clone}} \\
&d_j^{\mathrm{DTW}} = \min_{\pi} \sum_{(p,q) \in \pi} \norm{\mathbf{e}_p^{\real} - \mathbf{e}_q^{\clone}}_2 \quad \text{where} \quad \pi \in \mathcal{A}(T_j^{\real}, T_j^{\clone}) \\
&\bar{d}_j = d_j^{\mathrm{DTW}} / A_{\max}^i \quad \text{(Normalized distance)} \\
&A_{\max}^i = \max_{t} |u_i(t)| \quad \text{(Peak amplitude)}
\end{align}

\noindent where $\mathcal{A}(m,n)$ denotes the set of admissible warping paths satisfying:
\begin{itemize} 
    \item Boundary conditions: $\pi(1) = (1,1),\, \pi(K) = (m,n)$
    \item Monotonicity: $p_{k+1} \geq p_k,\, q_{k+1} \geq q_k$
    \item Step size: $(p_{k+1} - p_k, q_{k+1} - q_k) \in \{(1,0),(0,1),(1,1)\}$
\end{itemize}

\subsection{Statistical Modeling}
We model the distance distributions for each class:
\begin{align}
\mathcal{D}_{\class} &= \{\bar{d}_j : y_j = \class\} \quad \text{for} \quad \class \in \{\correct, \incorrect\} \\
F_{\class}(x) &= \mathbb{P}(\bar{d} \leq x \mid \class) = |\mathcal{D}_{\class}|^{-1} \sum_{d_k \in \mathcal{D}_{\class}} \mathbb{I}(d_k \leq x) \\
\tau_{\class} &= \inf \bigl\{ x : F_{\class}(x) \geq 0.9 \bigr\} \quad \text{(90th percentile threshold)}
\end{align}

\subsection{Runtime Detection}
For new utterance $u^*$ and synthesized clone $\hat{u}^*$:
\begin{align}
\bar{d}_j^* &= \frac{1}{A_{\max}^*} \min_{\pi} \sum_{(p,q) \in \pi} \norm{ \Psi(u^*)_p - \Psi(\hat{u}^*)_q }_2 \\
p_{\class}^j &= F_{\class}(\bar{d}_j^*) \quad \text{(Empirical CDF)} \\
\delta_{\class}^j &= |p_{\class}^j - 0.5| \quad \text{(Median deviation)} \\
D_j^* &= \begin{cases} 
    \correct & \text{if } \delta_{\correct}^j < \delta_{\incorrect}^j \\
    \incorrect & \text{otherwise}
\end{cases} \\
\hat{y}_j &= \begin{cases} 
    \text{CORRECT} & \text{if } (D_j^* = \correct) \land (\bar{d}_j^* \leq \tau_C) \\
    \text{INCORRECT} & \text{if } (D_j^* = \incorrect) \land (\bar{d}_j^* \geq \tau_I) \\
    \text{AMBIGUOUS} & \text{otherwise}
\end{cases}
\end{align}

\subsection{Theoretical Basis}
The decision rule follows from statistical distribution analysis:
\begin{itemize}
    \item \textbf{Distribution Selection}: Minimizes $\delta_{\class}^j$ to identify the most probable underlying distribution
    \item \textbf{Thresholding}: Uses class-specific thresholds $\tau_{\class}$ to handle distribution skewness
    \item \textbf{Ambiguous Region}: Defined where $\bar{d}_j^* \in (\tau_C, \tau_I)$ requires further analysis
\end{itemize}

==> methods_v1.tex <==
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\real}{\mathrm{real}}
\newcommand{\clone}{\mathrm{clone}}
\newcommand{\correct}{\mathrm{correct}}
\newcommand{\incorrect}{\mathrm{incorrect}}

\subsection{Data Preparation}

Let $\mathcal{U} = \{u_i\}_{i=1}^N$ be a corpus of real speech utterances with TextGrid annotations. Each utterance $u_i$ generates a synthesized clone $\hat{u}_i = V(u_i)$ via TTS system $V$. For each word $w_j$ in utterance $u_i$, we have a ground truth label $y_j \in \{\correct, \incorrect\}$, denoting if the pronunciation is correct or not.

Load real utterances \(U=\{u_i\}\) with TextGrids format and their TTS clones \(\hat U=\{\hat u_i\}\).
% For each \((u_i,\hat u_i)\), extract word spans
% % \[
% %   \{(w_j,\,[s_j^{\mathrm{real}},e_j^{\mathrm{real}}],\,[s_j^{\mathrm{clone}},e_j^{\mathrm{clone}}])\}.
% % \]
% \begin{equation}
%   \bigl\{\,\bigl(w_j,\,[s_j^{\mathrm{real}},e_j^{\mathrm{real}}],\,[s_j^{\mathrm{clone}},e_j^{\mathrm{clone}}]\bigr)\bigr\}.
% \end{equation}
    \subsection{Word Alignment}
    For each pair $ (u_i,\hat u_i) $, extract the set of word alignments:
    \begin{equation}
      \bigl\{\, \bigl( w_j, [s_j^{\mathrm{real}}, e_j^{\mathrm{real}}], [s_j^{\mathrm{clone}}, e_j^{\mathrm{clone}}] \bigr) \mid j = 1, \ldots, n_i \,\bigr\},
    \end{equation}
    where $ n_i $ is the number of words in the utterance, $ w_j $ is the $ j $-th word, and $ [s_j^{\mathrm{real}}, e_j^{\mathrm{real}}] $ and $ [s_j^{\mathrm{clone}}, e_j^{\mathrm{clone}}] $ are the start and end times of $ w_j $ in the real and clone utterance, respectively.


\subsection{Feature Extraction}
Compute 13-dimensional mel frequency cepstral coefficients (MFCC) envelopes \cite{itsp2022} \(E_j^{\mathrm{real}}\), \(E_j^{\mathrm{clone}}\) over each span.

\vspace{-1\baselineskip}
\subsection{Distance Computation}
Use dynamic time warping DTW to get  

\begin{equation}
  d_j^{\mathrm{DTW}}
    = \min_{\pi}\sum_t \bigl\lVert e_{j,t}^{\mathrm{real}}
    - e_{j,\pi(t)}^{\mathrm{clone}}\bigr\rVert,
  \quad
  \bar d_j = \frac{d_j^{\mathrm{DTW}}}{\max_t \bigl|u_i(t)\bigr|}.
\end{equation}


% \begin{equation}\label{eq:dtw}
%   d_j^{\mathrm{DTW}}
%     = \min_{\pi}\sum_t \bigl\lVert e_{j,t}^{\mathrm{real}}
%       - e_{j,\pi(t)}^{\mathrm{clone}}\bigr\rVert,
%   \quad
%   \bar d_j = \frac{d_j^{\mathrm{DTW}}}{\max_t \lvert u_i(t)\rvert}.
% \end{equation}


\vspace{-1\baselineskip}
\subsection{Threshold Calculation}
From all training distances split by true label,
\(\{\,\bar d_j : \text{correct}\}\) and \(\{\,\bar d_j : \text{incorrect}\}\),
compute class‐specific thresholds:
\begin{equation}
  \tau_C = \mathrm{Percentile}\bigl(\{\bar d_j\}_{\mathrm{correct}},\,90\%\bigr),
  \quad
  \tau_I = \mathrm{Percentile}\bigl(\{\bar d_j\}_{\mathrm{incorrect}},\,90\%\bigr).
\end{equation}


\vspace{-1\baselineskip}
\subsection{Distribution Selection}
For each new distance \(\bar d_j\), compute its empirical CDF in each class:
% \[
%   p_C = F_{\text{correct}}(\bar d_j), 
%   \quad
%   p_I = F_{\text{incorrect}}(\bar d_j).
% \]
\begin{equation}
  p_C = F_{\mathrm{correct}}(\bar d_j),
  \quad
  p_I = F_{\mathrm{incorrect}}(\bar d_j).
\end{equation}

Measure distance from the median (0.5):
% \[
%   \delta_C = \bigl|p_C - 0.5\bigr|,\quad
%   \delta_I = \bigl|p_I - 0.5\bigr|.
% \]
\begin{equation}
  \delta_C = \bigl|p_C - 0.5\bigr|,\quad
  \delta_I = \bigl|p_I - 0.5\bigr|.
\end{equation}

Choose the distribution whose center it’s closest to:
% \[
%   D^* = 
%   \begin{cases}
%     \text{correct}, & \delta_C < \delta_I,\\
%     \text{incorrect}, & \text{otherwise.}
%   \end{cases}
% \]
\begin{equation}
  D^* =
  \begin{cases}
    \text{correct},   & \delta_C < \delta_I,\\
    \text{incorrect}, & \text{otherwise.}
  \end{cases}
\end{equation}

\vspace{-1\baselineskip}
\subsection{Runtime Detection}
For a new utterance \(u\): synthesize \(\hat u = V(u)\), repeat steps 2–4 to get each \(\bar d_j\), then:
\begin{itemize}
  \item Select threshold \(\tau^* = \begin{cases}
      \tau_C, & D^*=\text{correct},\\
      \tau_I, & D^*=\text{incorrect},
    \end{cases}\)
  \item Assign
  % \[
  %   \hat y_j =
  %   \begin{cases}
  %     \text{CORRECT}, & D^*=\text{correct}\ \land\ \bar d_j \le \tau_C,\\
  %     \text{INCORRECT}, & D^*=\text{incorrect}\ \land\ \bar d_j \ge \tau_I,\\
  %     \text{AMBIGUOUS}, & \text{otherwise}.
  %   \end{cases}
  % \]
  \begin{equation}
  \hat y_j =
  \begin{cases}
    \text{CORRECT},   & D^*=\text{correct}\ \land\ \bar d_j \le \tau_C,\\
    \text{INCORRECT}, & D^*=\text{incorrect}\ \land\ \bar d_j \ge \tau_I,\\
    \text{AMBIGUOUS}, & \text{otherwise}.
  \end{cases}
\end{equation}

\end{itemize}
